Semi-Online Bipartite Matching

In this paper we introduce the \emph{semi-online} model that generalizes the classical online computational model. The semi-online model postulates that the unknown future has a predictable part and an adversarial part; these parts can be arbitrarily interleaved. An algorithm in this model operates as in the standard online model, i.e., makes an irrevocable decision at each step. We consider bipartite matching in the semi-online model, for both integral and fractional cases. Our main contributions are competitive algorithms for this problem that are close to or match a hardness bound. The competitive ratio of the algorithms nicely interpolates between the truly offline setting (no adversarial part) and the truly online setting (no predictable part).

==> missing_proofs_private.tex <==
\section{Proofs}

%%%%%%%%%%%%%%%%%%%%%% START OF COMMENTED BIG PROOF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse

\subsection{Proof of Theorem \ref{thm:algo-non-agnostic}}
\label{sec:proof-alg1}

In the analysis, we use the following folklore fact about maximum matchings, which we prove for the sake of completeness:
\begin{proposition}\label{prop:submatching}
Let $I$ be a bipartite graph with bipartition $A\cup B$ and let $A'\subseteq A$. Let $J$ be the induced subgraph of $I$ with node set $A'\cup B$. There exists a maximum matching $X$ of $I$ for which the restriction $X\cap E(J)$ to $J$ is a maximum matching of $J$.
\end{proposition}

\begin{proof}
Let $X$ be the maximum matching of $I$ with the minimum number of edges in $J$. Let $Y$ be a maximum matching of $J$. Assume, for the sake of contradiction, that $|X\cap E(J)| < |Y|$. Since $|X\cap E(J)| < |Y|$, some connected component $P$ of the edge set $X\cup Y$ has the property that $|P\cap X\cap E(J)| < |P\cap Y|$. If $P$ is a cycle or even-length path, augmenting the matching $X$ with $P$ results in a maximum matching of $I$ with strictly more edges than $X$ in $J$, a contradiction. Therefore, $P$ must be an odd-length path.

$P$ must have its endpoint edge(s) in $X$, as otherwise augmenting $X$ with $P$ would result in a larger matching of $I$. No non-endpoint node of $P$ can be in $A\setminus A'$, because each non-endpoint node of $P$ is incident with some edge in $J$. Since $P$ has odd length, its endpoints cannot both be in the same bipart. $P$ cannot entirely be contained in $J$, as otherwise augmenting $Y$ with $P$ would result in a larger matching in $J$. Therefore, $P$ has exactly one endpoint node $x$ outside of $A'\cup B$ and the subpath $P\setminus \{x\}$ is entirely contained in $J$. $P\setminus \{x\}$ is a path with even length with $|(P\setminus \{x\})\cap X\cap E(J)| = |(P\setminus \{x\})\cap Y|$. Therefore, $|P\cap X\cap E(J)| = |P\cap Y|$, a contradiction. In particular, $|X\cap E(J)| = |Y|$, so $X$ is a maximum matching whose restriction to $J$ is maximum.
\end{proof}

We now outline the analysis of our algorithm. For simplicity in this paragraph, assume that $G$ has a perfect matching. For the purposes of analysis, we maintain a matching $M^*$ over time. This matching starts out as a perfect matching. The crux of the argument for lower bounding the size of the $\mathcal D_{adv}$ matching is in showing that the number of nodes in $V_A$ that $M^*$ matches decreases by at most 1 during every iteration. This is shown using an augmenting path argument. When $G$ does not have a perfect matching, we show that $M^*$ decreases by a smaller amount in expectation.

Before formalizing this intuition, we define some more notation that we use in the proof. We start by defining the sequence of matchings $\{M_i^*\}_i$. By definition of each $H_i$, $H_{|U|-\nu(H)}$ has a matching with size $\nu(H)$, so the maximum matching will have this size. Therefore, we just need to lower bound the expected size of some matching in $G$ that contains the sampled matching. By definition of $u_i$, there is some matching $M_i$ in $H_i$ with size at least $\nu(H)$. Construct $M_i^*$ in $G$ as follows:

\begin{enumerate}
\item Let $M_0^*$ be a maximum matching in $G$ for which $M_0^*\cap H$ is a maximum matching of $H$ (exists by Proposition \ref{prop:submatching}).
\item For $i=1,2,\hdots,|U|-\nu(H)$
	\begin{enumerate}
    \item If $M_{i-1}^*$ does not match the node $u_i$, let $L_i^*\gets M_{i-1}^*$.
    \item Otherwise, let $F \gets M_{i-1}^*\cup M_i$. $F$ is a union of paths and cycles and $u_i$ is the endpoint of one path $P_i$ in $F$ (since $M_i$ does not match $u_i$ and $M_{i-1}^*$ does). Obtain $L_i^*$ by augmenting $M_{i-1}^*$ with the path $P_i$.
    \item If $u_i$ is matched by the online phase to an edge $e_i$ with online endpoint $x_i\in V_A$ and $x_i$ is incident with an edge $f_i\in L_i^*$, let $M_i^* \gets L_i^*\setminus \{f_i\}$.
    \item Otherwise, let $M_i^*\gets L_i^*$.
    \end{enumerate}
\end{enumerate}

Let $k_i$ denote the number of reserved nodes from the set $\{u_1, \ldots, u_i\}$ that are matched by the online phase.
Let $d_i$ denote the number of nodes $u_k$ with $k\le i$ for which both (a) $M_{k-1}^*$ matches $u_k$ and (b) $P_k$ has odd length.

We now prove some structural properties of the above matchings that will be helpful in proving the main theorem. Let $M_i'$ and $L_i'$ be the restrictions of the matchings $M_i^*$ and $L_i^*$ to $H$ respectively. We start by showing that these matchings are all maximum matchings in $H$:

\begin{proposition}\label{prop:greedy-pred}
$|M_i'| = |L_i'| = \nu(H)$ for all $i\ge 1$ and $|M_0'| = \nu(H)$.
\end{proposition}

\begin{proof}
We prove this by induction on $i$. For the base case, it suffices to show that $|M_0'| = \nu(H)$. This is true by definition of the matching $M_0^*$ (see Proposition \ref{prop:submatching}). Now, for $i\ge 1$ assume that $|M_{i-1}'| = \nu(H)$.

We first show that $|L_i'| = \nu(H)$. If $M_{i-1}^*$ does not match $u_i$, $L_i' = M_{i-1}'$ and $|L_i'| = |M_{i-1}'| = \nu(H)$ by the inductive hypothesis. Otherwise, $|M_{i-1}'|$ (by the inductive hypothesis) and $|M_i|$ (by definition of $M_i$) are both maximum matchings in $H$.

We now show that $P_i\cap H$ is the disjoint union of paths with even length. Suppose, for the sake of contradiction, that some connected component of $P_i\cap H$ is a path with an odd number of edges. The edges of $Q$ alternate between edges in $M_i$ and edges in $M_{i-1}'$. Since $Q$ has odd length, its endpoint edges must either both belong to $M_i$ or both belong to $M_{i-1}'$. If they both belong to $M_i$, then augmenting the matching $M_{i-1}'$ with $Q$ increases its size, contradicting the fact that $M_{i-1}'$ is a maximum matching in $H$. If the endpoint edges of $Q$ both belong to $M_{i-1}'$, then augmenting the matching $M_i$ with $Q$ increases its size, contradicting the fact that $M_i$ is a maximum matching in $H$. In both cases, we obtained a contradiction, so all components of $P_i\cap H$ must contain an even number of edges.

One can equivalently obtain $L_i'$ by augmenting $M_{i-1}'$ with all paths in $P_i\cap H$. Since all paths in $P_i\cap H$ have even length, $|L_i'| = |M_{i-1}'| = \nu(H)$, as desired.

Secondly, we show that $|M_i'| = \nu(H)$. This holds because $f_i$, if it exists, is not incident with any nodes in $V_P$. Therefore, $M_i' = L_i'$, as desired. This completes the inductive step and yields the desired result.
\end{proof}

Next, we bound the size of $M^*$ as a whole. We prove both an upper and lower bound:
\begin{proposition}\label{prop:greedy-real-lower}
$|M_i^*| \ge \nu(G) - d_i - k_i$ for all $i\ge 0$.
\end{proposition}

\begin{proof}
We show this by induction. For $i = 0$, the result is true because $M_0^*$ is a maximum matching of $G$. For $i\ge 1$, assume that $|M_{i-1}^*| \ge \nu(G) - d_{i-1} - k_{i-1}$. $|L_i^*| < |M_{i-1}^*|$ only when the augmenting path $P_i$ has odd length and $M_{i-1}^*$ matches $u_i$, and in this case $|L_i^*| = |M_{i-1}^*| - 1$. Therefore, $|L_i^*| \ge |M_{i-1}^*| - (d_i - d_{i-1})$. Furthermore, $|M_i^*| \ge |L_i^*| - (k_i - k_{i-1})$ because $|M_i^*| < |L_i^*|$ only when $u_i$ is matched. Summing these two inequalities and applying the inductive hypothesis shows that

\begin{align*}
|M_i^*| &\ge |M_{i-1}^*| - (d_i - d_{i-1}) - (k_i - k_{i-1})\\
&\ge \nu(G) - d_{i-1} - k_{i-1} - (d_i - d_{i-1}) - (k_i - k_{i-1})\\
&= \nu(G) - d_i - k_i\\
\end{align*}

as desired. This completes the inductive step.
\end{proof}

\begin{proposition}\label{prop:greedy-real-upper}
$|M_i^*| \le \nu(G) - d_i$ for all $i\ge 0$.
\end{proposition}

\begin{proof}
Finally, we show that $|M_i^*|\le \nu(G) - d_i$ for all $i\ge 0$. This is trivially the case $i = 0$, so assume that $|M_{i-1}^*|\le \nu(G) - d_{i-1}$ for some $i > 1$. $u_i$ cannot be incident with an edge in $M_i$. This means that $P_i$ cannot both have odd length and have $M_i$ edges as endpoint edges. Therefore, $|L_i^*|\le |M_{i-1}^*|$. If $M_{i-1}^*$ matches $u_i$ and $P_i$ has odd length, then $|L_i^*| = |M_{i-1}^*| - 1$. Therefore, $|L_i^*|\le |M_{i-1}^*| - (d_i - d_{i-1})$. Furthermore, $|M_i^*|\le |L_i^*|$, so $|M_i^*|\le |M_{i-1}^*| - (d_i - d_{i-1})\le \nu(G) - d_i$, as desired.
\end{proof}

We now prove two properties which will be used to show that no edge chosen for the $\mathcal D_{adv}$ matching shares an edge with previously chosen ones:

\begin{proposition}\label{prop:greedy-collide-offline}
$M_i^*$ is not incident to the nodes $u_1,u_2,\hdots,u_i$ for each $i\ge 0$.
\end{proposition}

\begin{proof}
Clearly this is true for $M_0^*$, so assume for $i\ge 1$ that $M_{i-1}^*$ is not incident to the nodes $u_1,u_2,\hdots,u_{i-1}$. If $M_{i-1}^*$ does not match $u_i$, $M_i^* = M_{i-1}^*$ and we are done. Otherwise, recall that $M_i$ does not match $u_1,u_2,\hdots,u_i$ since it is a matching in the graph $H_i$. Therefore, the path $P_i$ does not have an endpoint in the set $\{u_1,\hdots,u_{i-1}\}$, so augmenting $M_{i-1}^*$ with $P_i$ removes the matching edge of $M_{i-1}^*$ that matches $u_i$. Therefore, $M_i^*$ does not match any of $u_1,\hdots,u_i$, as desired.
\end{proof}

\begin{proposition}\label{prop:greedy-collide-online}
$M_i^*$ is not incident with the nodes $x_1,x_2,\hdots,x_i$ for each $i\ge 0$.
\end{proposition}

\begin{proof}
We show this by induction. This is vacuous for $i = 0$. Assume the result for $M_{i-1}^*$. The matching $M_i$ is not incident with any nodes in $V_A$ by definition. Since $M_{i-1}^*$ is also not incident with the nodes $x_1,x_2,\hdots,x_{i-1}\in V_A$, $P_i$ does not contain any of the nodes $x_1,\hdots,x_{i-1}$ and $L_i^*$ is not incident with $x_1,x_2,\hdots,x_{i-1}$. Since $M_i^*\subseteq L_i^*$, $M_i^*$ is also not incident with $x_1,\hdots,x_{i-1}$. Since $x_i$ is only incident with $f_i$ in $L_i^*$, $M_i^*$ is also not incident with $x_i$. This completes the inductive step.
\end{proof}

We now lower bound the expected value of the random variable $k_i$. Before doing this, we upper bound the expected value of $d_i$, which plays a role in lower bounding $k_i$ as seen in Proposition \ref{prop:greedy-real-lower}. Let $D_i := \textbf{E}[d_i]$ and let $K_i := \textbf{E}[k_i]$. Before bounding $D_i$, we deal with the trickiest part:

\begin{proposition}\label{prop:greedy-di-prob}
$\Pr_{u_i}[M_{i-1}^* \text{ matches } u_i | u_1,u_2,\hdots,u_{i-1}] \le \frac{|M_{i-1}^*|}{|U| - i + 1}$ for all $i\ge 1$.
\end{proposition}

\begin{proof}
$u_i$ is chosen uniformly at random from $U_i$. Let $U_i'$ denote the subset of $U_i$ consisting of nodes that are incident with an edge in $M_{i-1}^*$. Then
$$\Pr_{u_i}[M_{i-1}^* \text{ matches } u_i | u_1,u_2,\hdots,u_{i-1}] = \frac{|U_i'|}{|U_i|}$$
By definition of $U_i$, $U_i$ contains all nodes left in $U$ that are not matched by $M_{i-1}^*$. Therefore, $|U_i| - |U_i'| = (|U| - i + 1) - |M_{i-1}^*|$ and
\begin{align*}
\frac{|U_i'|}{|U_i|} &= \frac{|U_i'|}{|U_i'| + (|U| - i + 1) - |M_{i-1}^*|}\\
&\le \frac{|M_{i-1}^*|}{|M_{i-1}^*| + (|U| - i + 1) - |M_{i-1}^*|}\\
&\le \frac{|M_{i-1}^*|}{|U| - i + 1}\\
\end{align*}
since $|U_i'|\le |M_{i-1}^*|$. This is the desired result.
\end{proof}

Now, we bound $D_i$:

\begin{proposition}\label{prop:greedy-di-bound}
$D_i\le \frac{\nu(G)i}{|U|}$ for all $i\ge 0$.
\end{proposition}

\begin{proof}
$d_{i+1} - d_i > 0$ only if $u_{i+1}$ is incident with $M_i^*$, in which case $d_{i+1} = d_i + 1$. Therefore,
$$\textbf{E}[d_{i+1}|u_1,u_2,\hdots,u_i] = \Pr_{u_{i+1}}[M_i^* \text{ matches } u_{i+1} | u_1,u_2,\hdots,u_i] + d_i$$
Therefore, by Propositions \ref{prop:greedy-di-prob} and \ref{prop:greedy-real-upper},
\begin{align*}
\textbf{E}[d_{i+1}|u_1,u_2,\hdots,u_i] &\le \frac{|M_i^*|}{|U| - i} + d_i\\
&\le \frac{\nu(G) - d_i}{|U| - i} + d_i\\
&\le \frac{\nu(G)}{|U| - i} + \left(1 - \frac{1}{|U| - i}\right)d_i\\
\end{align*}
By the tower law of conditional expectations,
\begin{align*}
D_{i+1} &= \textbf{E}[\textbf{E}[d_{i+1}|d_1,\hdots,d_i]]\\
&\le \frac{\nu(G)}{|U| - i} + \left(1 - \frac{1}{|U| - i}\right)D_i\\
&
\end{align*}
We now inductively show the desired result. $D_0 = 0$ by definition. For $i \ge 0$, assume that $D_i\le \frac{\nu(G)i}{|U|}$. Then,
\begin{align*}
D_{i+1} &\le \frac{\nu(G)}{|U| - i} + \left(1 - \frac{1}{|U| - i}\right)D_i\\
&\le \frac{\nu(G)}{|U| - i} + \left(1 - \frac{1}{|U| - i}\right)\frac{\nu(G)i}{|U|}\\
&= \frac{\nu(G)}{|U| - i} + \frac{\nu(G)i}{|U|} - \frac{\nu(G)i}{|U|(|U| - i)}\\
&= \frac{\nu(G)}{|U| - i} + \frac{\nu(G)i}{|U|} - \left(\frac{\nu(G)}{|U| - i} - \frac{\nu(G)}{|U|}\right)\\
&= \frac{\nu(G)(i+1)}{|U|}\\
\end{align*}
as desired.

\end{proof}

We are now ready to lower bound $K_i$:

\begin{proposition}\label{prop:greedy-ki-bound}
$K_i\ge (1 - 1/|U|)^i \left(\frac{(\nu(G) - \nu(H))i}{|U|} - \nu(G)\frac{i^2}{2|U|^2}\right)$
\end{proposition}

\begin{proof}
Let $S_{i+1}$ be the set of nodes in $U$ matched to nodes in $V_A$ by $M_i^*$ for each $i\ge 0$. By Propositions \ref{prop:greedy-real-lower} and \ref{prop:greedy-pred},
$$|S_{i+1}|\ge (\nu(G) - d_i - k_i) - \nu(H) = \nu(G) - \nu(H) - d_i - k_i$$
By Proposition \ref{prop:greedy-collide-offline}, $M_i'$ is a matching in $H_i$. By Proposition \ref{prop:greedy-pred}, $|M_i'| = \nu(H)$. Therefore, $S_{i+1}\subseteq U_{i+1}$. In particular, $$\Pr[u_{i+1}\in S_{i+1}|u_1,\hdots,u_i] = \frac{|S_{i+1}|}{|U_{i+1}|} \ge \max\left(\frac{\nu(G) - \nu(H) - d_i - k_i}{|U_{i+1}|},0\right)$$
If $u_{i+1}\in S_{i+1}$, then $u_{i+1}$ will be matched to some node $x_{i+1}$ in the matching produced by $\mathcal D_{adv}$, since $u_{i+1}$ is matched by $M_i^*$ to some node that, by Proposition \ref{prop:greedy-collide-online}, was not previously matched by the online algorithm. Therefore,

\begin{align*}
\textbf{E}[k_{i+1}|u_1,u_2,\hdots,u_i] &\ge \Pr[u_{i+1}\in S_{i+1}|u_1,u_2,\hdots,u_i] + k_i\\
&\ge \max\left(\frac{\nu(G) - \nu(H) - d_i - k_i}{|U_{i+1}|},0\right) + k_i\\
&\ge \frac{\nu(G) - \nu(H) - d_i - k_i}{|U|} + k_i\\
&= \frac{\nu(G) - \nu(H)}{|U|} - \frac{d_i}{|U|} + \left(1 - \frac{1}{|U|}\right)k_i\\
\end{align*}
By the tower rule of conditional expectations and Proposition \ref{prop:greedy-di-bound},

\begin{align*}
K_{i+1} &= \textbf{E}[k_{i+1}]\\
&= \textbf{E}_{u_1,\hdots,u_i}[\textbf{E}_{u_{i+1}}[k_{i+1}|u_1,u_2,\hdots,u_i]]\\
&\ge \textbf{E}\left[\frac{\nu(G) - \nu(H)}{|U|} - \frac{d_i}{|U|} + \left(1 - \frac{1}{|U|}\right)k_i \right]\\
&= \frac{\nu(G) - \nu(H)}{|U|} - \frac{D_i}{|U|} + \left(1 - \frac{1}{|U|}\right)K_i\\
&\ge \frac{\nu(G) - \nu(H)}{|U|} - \frac{\nu(G)i}{|U|^2} + \left(1 - \frac{1}{|U|}\right)K_i\\
\end{align*}
For all $k\ge 0$, let $K_k' := \frac{K_k}{(1 - 1/|U|)^k}$. Then $K_0' = 0$ and
$$K_{i+1}' \ge \frac{\nu(G) - \nu(H) - \nu(G)(i/|U|)}{|U|(1 - 1/|U|)^{i+1}} + K_i'$$
for all $i\ge 0$. Therefore,
$$K_i' \ge \sum_{j=0}^{i-1} \frac{\nu(G) - \nu(H) - \nu(G)(j/|U|)}{|U|(1 - 1/|U|)^{j+1}}$$
and

\begin{align*}
K_i &\ge \sum_{j=0}^{i-1} (1 - 1/|U|)^{i-j-1} \frac{\nu(G) - \nu(H) - \nu(G)(j/|U|)}{|U|}\\
&\ge (1 - 1/|U|)^i \sum_{j=0}^{i-1} \frac{\nu(G) - \nu(H) - \nu(G)(j/|U|)}{|U|}\\
&= (1 - 1/|U|)^i \left(\frac{(\nu(G) - \nu(H))i}{|U|} - \nu(G)\frac{i(i-1)}{2|U|^2}\right)\\
&\ge (1 - 1/|U|)^i \left(\frac{(\nu(G) - \nu(H))i}{|U|} - \nu(G)\frac{i^2}{2|U|^2}\right)\\
\end{align*}
as desired.

\end{proof}

Now that we have lower bounded the expected size of the matchings produced by both $\mathcal D_{pred}$ and $\mathcal D_{adv}$, we are ready to prove the main result:

\begin{proof}[Proof of Theorem \ref{thm:algo-non-agnostic}]
Since $k_{i+1}\ge k_i$ for all $i\ge 0$, $K_{|U| - \nu(H)} \ge K_{\delta |U|}$. By Proposition \ref{prop:greedy-ki-bound} and the definition of $\delta$, $K_{|U| - \nu(H)}\ge (1 - \delta)\frac{\delta^2}{2}\nu(G)$. Therefore, $\mathcal D_{adv}$ produces matchings with size at least $(\delta^2/2 - \delta^3/2)\nu(G)$ in expectation. $\mathcal D_{pred}$ produces matchings with size exactly $\nu(H) = (1 - \delta)\nu(G)$. By Proposition \ref{prop:greedy-collide-offline}, the union of these matchings is itself a matching in $G$. Therefore, the union is a matching in $G$ with size at least $(1 - \delta + \delta^2/2 - \delta^3/2)\nu(G)$ in expectation, as desired.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%% END OF COMMENTED BIG PROOF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi



%%%%%%%%%%%%%%%%%%%%%% START OF COMMENT - FRACTIONAL %%%%%%%%%%%%%%%%%%%%%
\iffalse
\subsection{Reconstructing a fractional matching: Proof of Lemma~\ref{lem:vee}}
\label{sec:reconstruction}
In this section, we describe how a fractional matching can be  reconstructed, using the technique of~\cite{vee2010matching}.

Recall that we are given a graph $H = (U, V, E)$, where $|U| = |V| = n$, which has a perfect matching. We may write the fractional matching problem as the following quadratic program.
\begin{align}
&\mbox{\ \ }\min \frac{1}{2}\sum_{(u,v)\in E} x_{uv}^2 \nonumber \\
\text{s.t. \ \ } 
	& \forall_u,\ \ \sum_{v\in\Gamma(u)} x_{uv} = 1 
    		\label{eqn:alpha}\\
	& \forall_v,\ \ \sum_{u\in\Gamma(v)} x_{uv} \leq 1
    		\label{eqn:beta}\\
    & \forall_{(u,v)\in E},\ \ \ 0 \leq x_{uv} \leq 1
    		\label{eqn:tau}
\end{align}
The objective here may be a little surprising. However, Constraint~\ref{eqn:alpha} guarantees that any feasible solution will have a matching of size $n$. The objective is chosen simply to make reconstructing the solution easy. We will see this in a moment.

Note that since there is a perfect matching, this optimization problem always has a feasible solution. Let's write out its KKT conditions. Let $\alpha_u$ be the dual for Constraint~\ref{eqn:alpha}, $\beta_v$ the dual for Constraint~\ref{eqn:beta}, and $\tau_{uv}^0, \tau_{uv}^1$ be the duals for Constraint~\ref{eqn:tau}. Letting $x^*$ denote the optimal solution, we have
\begin{align}
\forall_{(u,v)\in E},\ x^*_{uv}  - \alpha_u + \beta_v - \tau_{uv}^0 + \tau_{uv}^1 = 0 
	\label{eqn:primal}\\
\intertext{Complementary slackness:} 
\forall_u,\ 	\alpha_u \cdot \bigg(\sum_{v\in\Gamma(u)} x^*_{uv} - 1\bigg) = 0\\
\forall_v,\	\beta_v \cdot \bigg(\sum_{u\in\Gamma(v)} x^*_{uv} - 1\bigg) = 0
    			\label{eqn:comp_beta}\\
\forall_{(u,v)\in E},\	\tau_{uv}^0 \cdot x^*_{uv} = 0 = \tau_{uv}^1\cdot (x^*_{uv} - 1)
    			\label{eqn:comp_tau}\\
\text{with \ } \alpha_u, \beta_v, \tau_{uv}^0, \tau_{uv}^1 \ge 0\nonumber
\end{align}
Constraint~\ref{eqn:primal} can be rewritten as $x^*_{uv}  = \alpha_u - \beta_v + \tau_{uv}^0 - \tau_{uv}^1$. Inspecting this more carefully, note that if $0 < \alpha_u - \beta_v < 1$, then by complementary slackness (Constraint~\ref{eqn:comp_tau}), both $\tau_{uv}^0 = \tau_{uv}^1 = 0$. That is, $x^*_{uv} = \alpha_u - \beta_v$. On the other hand, if $\alpha_u - \beta_v < 0$, then since $x^*_{uv} \geq 0$, we must have $\tau_{uv}^0 = \beta_v - \alpha_u$. Hence, $x^*_{uv} = 0$. An analogous argument shows that if $\alpha_u - \beta_v > 1$, then $x^*_{uv} = 1$. Putting this together, we see
$$
x^*_{uv} = \min(\max(0, \alpha_u - \beta_v), 1)
$$
In other words, we can reconstruct $x^*_{uv}$ using only the $n$ dual $\alpha$ values and $n$ dual $\beta$ values. Wonderfully, we can do even better. Suppose we have only the $\alpha$ values. Given the neighborhood of any online node $v$, we can reconstruct the value of $x^*_{uv}$ for all $u$ in the neighborhood. By Constraint~\ref{eqn:comp_beta}, we have
\begin{align*}
\beta_v \cdot \bigg(\sum_{u\in\Gamma(v)} x^*_{uv} - 1\bigg) = 0\\
\beta_v \cdot \bigg(\sum_{u\in\Gamma(v)} \min(\max(0, \alpha_u - \beta_v), 1) - 1\bigg) = 0 %\\
%\text{Hence, either $\beta_v = 0$ or\ }
%\sum_{j\in\Gamma(i)} \min(\max(0, \alpha_u - \beta_v), 1) = 1
\end{align*}
Since we know all the $\alpha_u$, and $x_{uv} \leq 1$, we can solve this for $\beta_v$ (in linear time). Just solve the equation $\sum_{j\in\Gamma(i)} \min(\max(0, \alpha_u - z), 1) = 1$ for $z$ and set $\beta_v = \max(0, z)$.
In other words, given only the $\alpha$ dual values, we can reconstruct all the $x^*_{uv}$ using the structure of the graph.

Noting that we can solve this quadratic program in polytime (using the Ellipsoid Algorithm), we can find the dual values $\alpha_u$ in polytime, and Lemma~\ref{lem:vee} follows.

\fi
%%%%%%%%%%%%%%%%%%%%%% END OF COMMENT - FRACTIONAL %%%%%%%%%%%%%%%%%%%%%

\subsection{Fractional Matching: Proof of Theorem \ref{thm:fractional-matching}}\label{sec:fractional_matching_appendix}
As we noted earlier, if the realized graph were exactly as predicted, we would give the fractional assignment $x$ guaranteed in Lemma~\ref{lem:vee}, which has weight $n$. However, the fractional matching that is actually realized is somewhat different.
For each online node that arrives, we treat it the same whether it is adversarial or not. But we have a few cases to consider for analysis:
\begin{itemize}
\item Case 1: The online node $v$ is adversarial. In this case, we forfeit the entire weight of 1 in the matching. We may assign some fractional matching to incident edges. However, we count this is `excess' and do not credit it towards our total. In this way, we lose at most $\delta n$ total weight.
\item Case 2: The online node $v$ is not adversarial, but it has extra edges added through a random process. There are at most $\epsilon n$ such nodes in expectation. In this case, we treat them the same as adversarial. We forfeit the entire weight of 1, and ignore the `excess' assignment. This loses at most $\epsilon n$ total weight in expectation.
\item Case 3: The online node $v$ is as exactly as predicted. In this case, we correctly calculate $x_{uv}$ for each $u\in\Gamma(v)$. Further, we assign $x_{uv}$ to each edge, unless there was already `excess' there. Since we never took credit for this excess, we will take $x_{uv}$ credit now. So we do not lose anything in this case.
\item Case 4: The online node $v$ is as predicted, except each edge is removed with probability $\epsilon$ (and no edges are added). In this case, when we solve for $z$, we find a value that is bounded above by the true $z$. The reason is that in the predicted graph, we solved $\sum_{u\in\Gamma(v)} \min(\max(0, \alpha_u - z), 1) = 1$ for $z$ when computing $g$.
In the realized graph, this same sum has had some of its summands removed, meaning the solution in $z$ is at most what it was before. So the value of $\tilde{x}_{uv}$ that we calculate is at least $x_{uv}$ for all $u$ in the realized neighborhood. We take a credit of $x_{uv}$ for each of these, leaving the rest as excess. Note that we have assigned $0$ to each edge that was in the predicted graph but missing in the realized graph. Since each edge goes missing with probability $\epsilon$, this is a total of at most $\epsilon n$ in expectation.
\end{itemize}
So, the total amount we lose in expectation is $2\epsilon n + \delta n$. Since the matching in the predicted graph has weight $n$, the claim follows.
